DensePure: Understanding Diffusion Models towards Adversarial Robustness

Diffusion models have been recently employed to improve certified robustness through the process of denoising. However, the theoretical understanding of why diffusion models are able to improve the certified robustness is still lacking, preventing from further improvement. In this study, we close this gap by analyzing the fundamental properties of diffusion models and establishing the conditions under which they can enhance certified robustness. This deeper understanding allows us to propose a new method DensePure, designed to improve the certified robustness of a pretrained model (i.e. classifier). Given an (adversarial) input, DensePure consists of multiple runs of denoising via the reverse process of the diffusion model (with different random seeds) to get multiple reversed samples, which are then passed through the classifier, followed by majority voting of inferred labels to make the final prediction. This design of using multiple runs of denoising is informed by our theoretical analysis of the conditional distribution of the reversed sample. Specifically, when the data density of a clean sample is high, its conditional density under the reverse process in a diffusion model is also high; thus sampling from the latter conditional distribution can purify the adversarial example and return the corresponding clean sample with a high probability. By using the highest density point in the conditional distribution as the reversed sample, we identify the robust region of a given instance under the diffusion model's reverse process. We show that this robust region is a union of multiple convex sets, and is potentially much larger than the robust regions identified in previous works. In practice, DensePure can approximate the label of the high density region in the conditional distribution so that it can enhance certified robustness.

==> sections/abs.tex <==
Existing works view diffusion models as blackbox models and demonstrate that diffusion models can improve  certified robustness. However,  a theoretical understanding of how and under what conditions diffusion models are able to improve certified robustness is lacking. 
In this work, we theoretically analyze the fundamental properties of diffusion model in why and how it can enhance certified robustness and propose \name to improve the certified robustness of a standard model by properly using the diffusion  model based on these properties.
% In this work, we  delve into diffusion model and propose \name to improve the certified robustness of a standard classifier by properly using the off-the-shelf diffusion models based on our theoretical analysis.
% In this work, we  delve into diffusion model and propose \name to improve the certified robustness of a vanilla model by properly use the off-the-shelf diffusion model based on our theoretical analysis of diffusion models. 
% Theoretically, 
In theory, we prove that diffusion models purify the adversarial example back to the corresponding clean sample with a high probability, as long as the \textit{data} density of clean samples is sufficiently high. Furthermore, 
we characterize the conditional distribution of the reversed samples given the adversarial input, which is generated by the reverse process of the diffusion model. Using the highest density point in the conditional distribution, we identify the robust region of a given instance under the diffusion model reverse process. We find this robust region is a union of multiple convex sets, and is potentially much larger than the robust regions in previous works. 
% we characterize the conditional distribution of the reversed samples conditioned on the adversarial input. Using the highest density point in the conditional distribution, we characterize the robust region of a given instance under the diffusion model reverse process, which is a union of multiple convex sets and potentially much larger than the robust regions in previous works. 
Inspired by theoretical analyses, \name is designed to approximate the label of the high density manifold in the conditional distribution by incorporating two steps. \name (i) performs the reverse process of a diffusion model to obtain a sample of the posterior data distribution conditioned on the  (adversarial) input, and (ii) repeats such reverse process multiple times with majority vote  for final prediction. 
We conduct extensive experiments to demonstrate the effectiveness of \name by evaluating its certified robustness under given a standard model via randomized smoothing. We show that 
% \name achieves  76.6\% certified accuracy on CIFAR-10 under adversarial perturbations within  $L_2$ norm  0.25, an improvement of 3\% over prior methods. 
\name is consistently better than existing methods on ImageNet, 7\% improvement on average. 
% For instance, our method achieves 77\% certified accuracy within $L_2$ norm 0.5,  7\% improvement over prior methods.


==> sections/abs3.tex <==



\textbf{version 3}

Existing works demonstrate that diffusion models can improve certified robustness empirically.  However, the theoretical understanding of why diffusion models are able to improve the certified robustness is still lacking, preventing from further improvement.  

In this work, we theoretically  analyze why and how diffusion models can enhance certified robustness. Inspired by our theoretical analysis,  we propose \name to  improve the certified robustness of a standard model by properly using the diffusion  model. Specifically,  \name consists of the off-the-shelf diffusion model and standard classifier.  It repeatedly feeds the (adversarial) input into the reverse process of a diffusion model, following by a classifier, multiple times  and  uses majority vote for final prediction.  

% In this work, we  delve into diffusion model and propose \name to improve the certified robustness of a standard classifier by properly using the off-the-shelf diffusion models based on our theoretical analysis.
% In this work, we  delve into diffusion model and propose \name to improve the certified robustness of a vanilla model by properly use the off-the-shelf diffusion model based on our theoretical analysis of diffusion models. 
In theory, we  prove that diffusion models purify the adversarial example back to the corresponding clean sample with a high probability, as long as the \textit{data} density of clean samples is sufficiently high. Furthermore, 
we characterize the conditional distribution of the reversed samples given the adversarial input, which is generated by the reverse process of the diffusion model. Using the highest density point in the conditional distribution, we identify the robust region of a given instance under the diffusion model reverse process. We find this robust region is a union of multiple convex sets, and is potentially larger than the robust regions in previous works. 
% In practice, \name can approximate the label of the high density manifold in the conditional distribution 
% we characterize the conditional distribution of the reversed samples conditioned on the adversarial input. Using the highest density point in the conditional distribution, we characterize the robust region of a given instance under the diffusion model reverse process, which is a union of multiple convex sets and potentially much larger than the robust regions in previous works. 
% Inspired by theoretical analyses, \name is designed to approximate the label of the high density manifold in the conditional distribution by incorporating two steps. \name (i) performs the reverse process of a diffusion model to obtain a sample of the posterior data distribution conditioned on the  (adversarial) input, and (ii) repeats such reverse process multiple times with majority vote  for final prediction. 
We conduct extensive experiments to demonstrate the effectiveness of \name by evaluating its certified robustness under given a standard model via randomized smoothing. We show that 
% \name achieves  76.6\% certified accuracy on CIFAR-10 under adversarial perturbations within  $L_2$ norm  0.25, an improvement of 3\% over prior methods. 
\name is consistently better than existing methods on ImageNet, 7\% improvement on average. 
% For instance, our method achieves 77\% certified accuracy within $L_2$ norm 0.5,  7\% improvement over prior methods.


==> sections/abs_bak.tex <==
%\textbf{version 2}

Diffusion models have been recently employed to  improve certified robustness through the process of denoising.  However, the theoretical understanding of why diffusion models are able to improve the certified robustness is still lacking, preventing from further improvement.  
% However,  theoretical guarantees for the denoising process are so far  lacking. 
%preventing from further improvement.  
In this study, we close this gap by analyzing fundamental properties of diffusion models  and formally establish the conditions under which they are guaranteed to enhance certified robustness.  
This deeper understanding allows us to propose a new method   \namens,  designed to improve  certified robustness of a given model.   \name consists of multiple runs of denoising of perturbed sample (with different random seeds), which are then passed through the classifier of the given model, followed by majority voting of inferred labels to make the final prediction.  
%\name is inspired by our theoretical analysis, 
This design of using multiple runs of denoising is informed by our theoretical analysis of the conditional distribution of the denoised sample. % In this work, we  delve into diffusion model and propose \name to improve the certified robustness of a standard classifier by properly using the off-the-shelf diffusion models based on our theoretical analysis.
% In this work, we  delve into diffusion model and propose \name to improve the certified robustness of a vanilla model by properly use the off-the-shelf diffusion model based on our theoretical analysis of diffusion models. 
Specifically, when the \textit{data} density of a clean sample is high, its conditional density under the reverse process in a diffusion model is also high;  thus sampling from the latter conditional distribution can purify the adversarial example and return the corresponding clean sample with a high probability. 
% Because high density of clean samples is sufficient to high conditional density of them. 
By using the highest density point in the conditional distribution as the denoised sample, we identify the robust region of a given instance under the diffusion model's reverse process. We show that this robust region is a union of multiple convex sets, and is potentially much larger than the robust regions identified in previous works. 
In practice, \name can approximate the label of the high density region in the conditional distribution so that it can enhance certified robustness. 
% we characterize the conditional distribution of the reversed samples conditioned on the adversarial input. Using the highest density point in the conditional distribution, we characterize the robust region of a given instance under the diffusion model reverse process, which is a union of multiple convex sets and potentially much larger than the robust regions in previous works. 
% Inspired by theoretical analyses, \name is designed to approximate the label of the high density region in the conditional distribution by incorporating two steps. \name (i) performs the reverse process of a diffusion model to obtain a sample of the posterior data distribution conditioned on the  (adversarial) input, and (ii) repeats such reverse process multiple times with majority vote  for final prediction. 
We conduct extensive experiments to demonstrate the effectiveness of \name by evaluating its certified robustness  given a standard model via randomized smoothing. We show that 
% \name achieves  76.6\% certified accuracy on CIFAR-10 under adversarial perturbations within  $L_2$ norm  0.25, an improvement of 3\% over prior methods. 
\name is consistently better than existing methods on ImageNet, with 7\% improvement on average. 
% For instance, our method achieves 77\% certified accuracy within $L_2$ norm 0.5,  7\% improvement over prior methods.


==> sections/intro.tex <==


\section{Introduction}
1. diffusion model is good at removing adv noise based on observations
2. but it is unclear about the fundamental reason or sufficient conditions under which diffusion models can effectively remove adv noise
3. we theoretically analyze, xxxxx (2 conclusions) (intuition: the union of xxxx, better than rs under general cases)
4. in practice, we propose to leverage the majority vote to approximate such high density region and therefore improve the certified robustness
5. exp results .....

\weili{Should we emphasize more the certified robustness in the intro?}

Diffusion models have demonstrated powerful image generation ability recently \citep{Ho2020DDPM, Song2021ICLR} due to the iterative diffusion and denoising processes. Such models so far have achieved the state-of-art performance on sample quality \citep{dhariwal2021diffusion, vahdat2021score}, as well as effective mode coverage \citep{song2021maximum}. 
In particular, diffusion models usually consist of two processes: (i) a forward diffusion process that converts data to noise by gradually adding noise to the input, and (ii) a reverse generative process that starts from noise and generates data by denoising one step at a time~\citep{Song2021ICLR}. 

Given the natural denoising property of diffusion models, \emph{empirical} studies have been conducted to show that it is possible to leverage diffusion models to perform adversarial purification~\citep{nie2022diffusion,wu2022guided,carlini2022certified}. For instance, 
\citeauthor{nie2022diffusion} introduced a diffusion model based purification model  \textit{DiffPure}, which first added Gaussian noises to the adversarial sample to obtain a diffused sample (via diffusion process) and then solved a reverse stochastic differential equation (SDE) (via reverse process) to remove the adversarial perturbation to recover a ``clean" sample \bo{certification} . They showed that by carefully choosing the amount of Gaussian noises added during the diffusion process, the adversarial perturbations can be removed while preserving the true label semantics. \citet{carlini2022certified} instantiated the randomized smoothing approach with diffusion model to empirically show the non-trivial certified robustness. 


Despite the empirical success of diffusion models in removing adversarial perturbations, the theoretical understanding for such process is still lacking.
In this work, we aim to ask: \textit{What are the sufficient conditions under which a diffusion model is able to remove adversarial perturbation?} \textit{Is it possible to further improve the purification performance based on the fundamental properties of diffusion models?}

In particular, we theoretically prove that under mild conditions, with the diffusion model, an adversarial example will always be recovered back to the corresponding clean sample with high probability, as long as the data density of the clean samples is high enough.
% In particular, we theoretically prove that, with the diffusion model, an adversarial example will always be recovered back to the corresponding clean sample with high probability, as long as the data density of the clean samples is high enough.
\bo{maybe more result later}
% In particular, we theoretically prove that under mild conditions, with the diffusion model, an adversarial example will always be recovered back to the corresponding clean sample with high probability, as long as the data density of the clean samples is high enough.\bo{maybe more result later}
% In our work, we showed that the diffusion process is unnecessary for adversarial purification because it will only add extra noise to the adversarial sample. \bo{hmm, is this the motivation? or we want to explore why diffusion model would help remove adv noise?} \kj{Agreed, I think we can say something like our major contribution is coming up with a better framework using some criteria, and a minor but worth mentioning point is that it can even bypass the diffusion process, resulting in even better efficiency or something} 
Based on our theoretical analysis, we show that in fact the diffusion process itself is not necessary when leveraging diffusion models for adversarial purification. 
Instead, by sending the adversarial example directly through the reverse process of the diffusion model, we can obtain a better-recovered sample in terms of its distance to the corresponding clean sample. 
% Based on our theoretical analysis, we show that in fact the diffusion process itself is not necessary when leveraging diffusion models for adversarial purification. 
% Instead, by sending the adversarial example directly through the reverse process of the diffusion model, we can obtain a better recovered sample in terms of its distance to the corresponding clean sample. 
On the other hand, after the reverse process, we actually obtain a distribution instead of a deterministic sample, which is a posterior of the data distribution conditioned on the adversarial example. The above characteristics enable us to design a more effective adversarial purification pipeline \name.

% Concretely, \name incorporates two steps: (i) we first leverage the reverse process of the diffusion model to obtain a posterior data distribution conditioned on the input adversarial example, and (ii) then we take the point with the highest density in the obtained distribution as the ``clean'' sample.
Concretely, \name incorporates two steps: (i) we first solve the reverse stochastic differential equation (SDE) to obtain a posterior data distribution conditioned on the input adversarial example, and (ii) then we take the point with the highest density in the obtained distribution as the clean sample, approximated by taking the majority vote for the prediction on different reversed samples.
We show that the robust region for each true prototype under \name is the union of all convex robust sub-region for prototypes (i.e., high density region with the same label as the true prototype). We believe that this characterization has the potential to provide larger robustness radius for inputs, since it is able to connect different convex robust sub-regions together. In addition, based on our formal characterization of the robust regions, we show that the size of robust regions is affected by the relative density and between the clean sample and neighborhood samples with different labels, and the distance of true prototype to prototypes with different labels. The influence of these two factors is controlled by the timestamp we choose in the reverse process.


Moreover, we instantiate \name with the randomized smoothing algorithm~\citep{Cohen2019ICML} to evaluate the certified robustness in practice. 
% However, it is hard for \name to take the point with the highest density in reality since it requires a heavy computation.
However, it is hard for \name to exactly sample the point of the highest density in practice as it needs an enormous amount of samplings to make a confident estimation of the densities for all points in the sample space.
We propose to  leverage the \textit{majority vote} on the classifier's prediction among different reversed samples instead. 
Our pipeline is shown in Figure~\ref{pipeline}. 
% Given the randomized input sampled from $\mathcal{N}(x_0, \sigma)$, we first compute the time-step $t$ used for the reverse processing. We then repeatedly feed the randomized input into the reverse process of a pre-trained diffusion model and classifier to get the majority-voted label for certification.


 We conduct extensive experiments on ImageNet and CIFAR-10 datasets under different settings. We show that our method could achieve the new state-of-the-art \emph{certified} robustness without tuning any model parameters (off-the-shelf).\chaowei{give numbers later}
We noted that although we can characterize the robust region for an input, generally it is non-convex with (possible) infinite constraints, which makes it hard to find a deterministic certification method to provide the robustness radius (lower bound) for each true prototype. Therefore, we resort to the randomized certification method in \cite{Cohen2019ICML}. On the other hand, we also noted that highest density point locating in high-dimensional spaces requires a huge amount of sampling, which is impossible in practice because we have to solve a SDE for every sampling. As an alternative, we proposed a label majority voting step to approximate the highest density point locating step.

\vspace{-0.2in}
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\includegraphics[width=0.5\linewidth]{figures/}
\end{center}
% \vspace{-0.2in}
\caption{Pipeline of \name.}\label{pipeline}
\label{robustfigure}
\end{figure}


\textbf{\underline{Contributions.}}
\begin{itemize}[leftmargin=*]
W take the first step towards understanding the sufficient conditions of \textit{adversarial purification} with diffusion models. We prove that under constrained data density property, an adversarial example can be recovered back to the original clean sample with high probability via the reverse process of a diffusion model. 
% \bo{mention we analyze both perfect/non-perfect reverse process, etc}\zc{our framework cannot analyze non-perfect reverse process where the Gaussian structure is destroyed}
    \item Based on our analysis, we proposed \name, which is a state-of-art adversarial purification pipeline directly leveraging the reverse process of a pre-trained diffusion model and a highest density point locating step.
    \item We characterized the robust region for each point under \name.
    \item We demonstrated state-of-art performance of \name on xxxx
\end{itemize}







==> sections/intro2.tex <==


\section{Introduction}
% 1. diffusion model is good at removing adv noise based on observations
% 2. but it is unclear about the fundamental reason or sufficient conditions under which diffusion models can effectively remove adv noise
% 3. we theoretically analyze, xxxxx (2 conclusions) (intuition: the union of xxxx, better than rs under general cases)
% 4. in practice, we propose to leverage the majority vote to approximate such high density region and therefore improve the certified robustness
% 5. exp results .....

% \weili{Should we emphasize more the certified robustness in the intro?}

Diffusion models have demonstrated powerful image generation ability recently \citep{Ho2020DDPM, Song2021ICLR} due to the iterative diffusion and denoising processes. Such models so far have achieved state-of-art performance on sample quality \citep{dhariwal2021diffusion, vahdat2021score}, as well as effective mode coverage \citep{song2021maximum}. 
In particular, diffusion models usually consist of two processes: (i) a forward diffusion process that converts data to noise by gradually adding noise to the input, and (ii) a reverse generative process that starts from noise and generates data by denoising one step at a time~\citep{Song2021ICLR}. 

Given the natural denoising property of diffusion models, \emph{empirical} studies have been conducted to show that it is possible to leverage diffusion models to perform adversarial purification~\citep{nie2022diffusion,wu2022guided,carlini2022certified}. For instance, 
\citeauthor{nie2022diffusion} introduced a diffusion model based purification model  \textit{DiffPure}, which first added Gaussian noises to the adversarial sample to obtain a diffused sample (via diffusion process) and then solved a reverse stochastic differential equation (SDE) (via reverse process) to remove the adversarial perturbation to recover a ``clean" sample. They showed that by carefully choosing the amount of Gaussian noises added during the diffusion process, the adversarial perturbations can be removed while preserving the true label semantics. \citet{carlini2022certified} instantiated the randomized smoothing approach with the diffusion model to remove added Gaussian noise, so as to provide certified robustness which offers a provable guarantee that a clean model's prediction is robust to  $L_2$-norm bounded adversarial example.


% Despite the empirical success of diffusion models in removing adversarial perturbations, the theoretical understanding for such process is still lacking.
Despite the success of diffusion models in removing adversarial perturbations, theoretical understanding is still lacking. Thus, natural questions emerge: \textit{What are the sufficient conditions under which a diffusion model is able to remove adversarial perturbation?} \textit{Is it possible to further improve the purification performance based on the fundamental properties of diffusion models?}

In this work,  we theoretically prove that with the diffusion model based adversarial purification pipelines~\citep{nie2022diffusion}, an adversarial example will always be recovered back to the sample with the ground-truth label with high probability, as long as the data density of the sample with the ground-truth label is high enough. 
% Based on our theoretical analysis, we propose an effective pipeline, \name.
% we achieve two goals: (1) we theoretically prove that with the diffusion model based adversarial purification pipelines~\citep{nie2022diffusion}, an adversarial example will always be recovered back to the sample with the ground-truth label with high probability, as long as the data density of the sample with the ground-truth label is high enough; and (2) Based on the theoretical analysis, 
% In this work, we theoretically prove that with the diffusion model based adversarial purification pipelines~\citep{nie2022diffusion}, an adversarial example will always be recovered back to the sample with the ground-truth label with high probability, as long as the data density of the sample with the ground-truth label is high enough. Based on the theoretical analysis, we propose an effective pipeline, \name, to improve adversarial robustness compared to \citep{nie2022diffusion}, which incorporates two-step : (i) we first use the reverse process to obtain a posterior data distribution conditioned on the input adversarial example, and (ii) then we take the point with the highest density in the obtained distribution as the clean sample, approximated by taking the majority vote for the prediction on different reversed samples in practical.   
% \bo{do we want to use clean sample or sample with the ground-truth label here?}
Specifically, when we feed an adversarial example into the reverse process of the diffusion model, the reverse process generates a conditional distribution over the trained data manifold based on the given adversarial sample. When we explicitly characterize the above obtained conditional density function, its formulation implies that the manifold with the ground-truth label of the given adversarial example has a higher density than the manifolds with other labels. Thus, If we use the highest density point in the conditional distribution as the reversed sample, it is more likely to predict the reversed sample as ground-truth compared to directly feeding the adversarial examples into the classifier. Moreover, if the density of the ground-truth label is high enough, the reversed example will always be predicted as the ground-truth label.  


The above analysis inspires us to propose the pipeline, \name. \name incorporates two steps:  (i) first using the reverse process of the diffusion model to obtain a posterior data distribution conditioned on the input adversarial input; and (ii) taking the point with the highest density in the obtained distribution as the purified sample for prediction. 
In practice,  the second step is, however, hard to be implemented as it needs an enormous amount of samplings to confidently estimate the densities in the whole sample space. To address this problem, we use \textit{majority vote} to reduce the heavy computations.  
% for the prediction on different reversed samples. 
In particular,  given an adversarial input, we repeatedly feed it into the reverse process of the diffusion model to get multiple reversed examples and feed them into the classifier to get the predictions. We then apply the \textit{majority vote} on such predictions to get the final predicted label. We prove that the reverse process of the diffusion model will generate samples in the surrounding neighborhood of the manifold with ground-truth label  with a high probability. This implies that \textit{majority vote} will high likely output the label of the highest density point.
% , which is also the ground-truth label.


Additionally, we also analyze the robustness radius of \name. We characterize the robustness region of any data manifolds with the ground-truth label such that all adversarial samples will be classified correctly. We identify that the robustness region of \name is a union of multiple convex sets, each surrounding a manifold with the ground-truth label. Compared to the robustness radius of previous work~\cite{Cohen2019ICML}, only focusing on the neighborhood of {\em one} manifold with the ground-truth label, \name will have the potential to provide a larger robustness radius. Moreover, the characterization implies that the size of robustness regions is affected by the relative density and the distance of data manifolds with the ground-truth label and manifolds with other labels. The influence of these two factors is controlled by the timestamp we choose in the reverse process.  \chaowei{Not sure whether we need the last two sentences. I find it not strictly connected with the previous sentences. It seems that we miss something in the middle. }
% The influence of these two factors is controlled by the timestamp we choose in the reverse process. 


% For clarity, we call the samples in the data manifold as prototypes, which are used to train the classifier. An adversarial sample adds perturbation to a prototype so that it locates outside of the manifold and make the classifier fail. We call the label corresponding to the attacked prototype as the ground-truth label, and prototypes with the ground-truth label as true prototypes. The reverse process of the diffusion model generates a conditional distribution over prototypes based on the given adversarial sample. We explicitly characterized the conditional density function whose formulation implies that the true prototypes have higher density than other prototypes. 
% On the other hand, these prototypes can be recognized well by classifiers train on the data manifold.

% We show that prototypes near the adversarial sample not only have high density in the conditional distribution, but also keep the label semantics of the adversarial sample. \kj{This sentence needs more reasoning} In other words, the reverse process will highly likely to sample a true prototype. 


% For further theoretical analysis, we use the highest density point in the conditional distribution as the clean sample, 
% % to remove randomness, 
% who will be sent to the classifier to predict the ground-truth label. The clean sample will locate in the data manifold and thus the classification outcome will be much more reliable than directly classifying the adversarial sample.
% In addition to the robustness radius studied in previous works, we characterize the robustness region of any true prototype such that all adversarial samples will be classified correctly. We show the robustness region is a union of convex sets, each surrounding a true prototype, and this characterization (the connection of convex sets) has the potential to provide a larger robustness radius than other certification methods \zc{cite} only focusing on the neighborhood of one true prototype. Moreover, the characterization also implies that the size of robustness regions is affected by the relative density and the distance of true prototypes to other prototypes. The influence of these two factors is controlled by the timestamp we choose in the reverse process. 

% In this work, we theoretically characterize the robustness region for a sample with the ground-truth label such that if the adversarial sample lies within the robustness region, the highest density point in the conditional distribution will have the ground-truth label. We further show that this robustness region is the union of all convex robustness sub-regions surrounding samples with the ground-truth label. We note that previous works \zc{which to cite} typically focus on investigating the robustness radius in the neighborhood of the only sample, similar to the robustness convex sub-region we established. We believe our characterization has the potential to provide a larger \kj{needs a comparison target} robustness radius compared to the previous work, since it is able to connect different convex robustness sub-regions together\zc{graph}. In addition, the characterization also implies that the size of robustness regions is affected by the relative density and the distance of true prototype \kj{this is the first time we see the term ``prototype'', and we should give it a definition or say it's equivalent to a clean sample with ground-truth label} to prototypes with different labels. The influence of these two factors is controlled by the timestamp we choose in the reverse process. 

% \kj{Not the best way to say it, but probably a way to reduce the repetitiveness in some sentences.\\
% In addition to the robustness radius studied in previous works, we characterize the robustness region of a sample with a ground-truth label such that all adversarial samples within will be classified with the ground-truth label. We further show the robustness region is a union of convex sets, each surrounding a sample with the same ground-truth label as the current sample, and this characterization (the connection of convex sets) has the potential to provide a large robustness radius.}


% Based on the above analysis, we design \name as shown in Figure~\ref{}. It incorporates with two steps: (i) we first use the reverse process of diffusion model to obtain a posterior data distribution conditioned on the input adversarial example; and (ii) then we take the point with the highest density in the obtained distribution as the clean sample. The second step is hard to implement in practice as it needs an enormous amount of samplings to make a confident estimation of the densities 
% % for all points 
% in the sample space. Thus, in practice, we feed the input adversarial example multiple time into the reverse process and leverage the \textit{majority vote} on the classifier's prediction among different reversed samples to approximate the true prediction. We prove that the reverse process of the diffusion model will generate samples in the surrounding neighborhood of the true prototypes with high probability. This implies that  \textit{majority vote} will high likely output the label of the highest density point, which is also the ground-truth label.


% \kj{Should we flip the order of this and the next paragraph?}




% approximated by taking the majority vote for the prediction on different reversed samples in practice. 

%%%%%%%
%%%%%%%
%%%%%%%
%%%%%%%
% In practice, it is challenging to exactly sample the point of the highest density in practice as it needs an enormous amount of samplings to make a confident estimation of the densities for all points in the sample space. Thus, we propose to leverage the \textit{majority vote} on the classifier's prediction among different reversed samples to approximate the true prediction. We proved that the reverse process of the diffusion model will generate samples in the surrounding neighborhood of the true prototype where it is more likely that the prototypes with the same label as the true prototype have the highest probability and one such prototype takes the highest density. In this case, \textit{majority vote} will output the label of the highest density point. \kj{Should we flip the order of this and the next paragraph?}

% The above analysis enables us to design a certifiably robust adversarial purification pipeline \name~ (Figure~\ref{pipeline}), which incorporates two steps: (i) we first solve the reverse stochastic differential equation (SDE) to obtain a posterior data distribution conditioned on the input adversarial example, and (ii) then we take the point with the highest density in the obtained distribution as the clean sample, approximated by taking the majority vote for the prediction on different reversed samples.
%%%%%%%
%%%%%%%
%%%%%%%
%%%%%%%

% In the literature, people are interested in the certified robustness radius, which can be obtained by finding the maximum inclined ball in the robustness region. However, this requires solving an infinite optimization problem due to the infinite number of constraints we use to form the robustness region. Without any restriction on the data distribution, we cannot obtain a certified robustness radius within finite time. Therefore, we resort to the randomized smoothing algorithm~\citep{Cohen2019ICML} to evaluate the certified robustness in practice.

We conduct extensive experiments on ImageNet and CIFAR-10 datasets under different settings to evaluate the certifiable robustness of \name. In particular, we follow the setting from \citet{carlini2022certified} and rely on  randomized smoothing to certify robustness to adversarial perturbations bounded in the $\mathcal{L}_2$-norm.   We show that \name~ achieves the new state-of-the-art \emph{certified} robustness on the clean model without tuning any model parameters (off-the-shelf). \name obtains significantly better certified robustness results  xxxx
% We noted that although we can characterize the robust region for an input, generally it is non-convex with (possible) infinite constraints, which makes it hard to find a deterministic certification method to provide the robustness radius (lower bound) for each true prototype. Therefore, we resort to the randomized certification method in \cite{Cohen2019ICML}. On the other hand, we also noted that highest density point locating in high-dimensional spaces requires a huge amount of sampling, which is impossible in practice because we have to solve a SDE for every sampling. As an alternative, we proposed a label majority voting step to approximate the highest density point locating step.

% \vspace{-0.2in}
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\includegraphics[width=0.5\linewidth]{figures/}
\end{center}
% \vspace{-0.2in}
\caption{Pipeline of \name.}\label{pipeline}
\label{robustfigure}
\end{figure}

% \textbf{\underline{Technical Contributions.}}
% In this paper, we take the first step towards understanding the sufficient conditions of \textit{adversarial purification} with diffusion models.
% We make contributions on both theoretical
% and empirical fronts.
% %%\vspace{-0.5em}
% \begin{itemize}[leftmargin=*]
%     \item We proved that under constrained data density property, an adversarial example can be recovered back to the clean sample with high probability via the reverse process of a diffusion model. 
%     \item By choosing the highest density point in the conditional distribution generated by the reverse process of the diffusion model as the ``clean" sample, we theoretically characterized the robustness region for adversarial samples such that the ``clean" sample has the correct label.
%     \item Based on our analysis and with some compromise due to the computation complexity, we proposed \name in practice, which is a state-of-art adversarial purification pipeline directly leveraging the reverse process of a pre-trained diffusion model and a majority vote step.
%     \item We demonstrated state-of-art performance of \name on xxxx
% \end{itemize}

\textbf{\underline{Technical Contributions.}}
In this paper, we take the first step towards understanding the sufficient conditions of \textit{adversarial purification} with diffusion models.
We make contributions on both theoretical
and empirical fronts.
%%\vspace{-0.5em}
\begin{itemize}[leftmargin=*]
    \item We prove that under constrained data density property, an adversarial example can be recovered back to the original clean sample with high probability via the reverse process of a diffusion model.
    \item Based on our analysis, we proposed \name, which is a state-of-art adversarial purification pipeline directly leveraging the reverse process of a pre-trained diffusion model and a highest density point locating step.
    \item We characterized the robust region for each point under \name.
    \item We demonstrated state-of-art performance of \name~ on xxxx
\end{itemize}


==> sections/intro2_bak.tex <==


\section{Introduction}
% 1. diffusion model is good at removing adv noise based on observations
% 2. but it is unclear about the fundamental reason or sufficient conditions under which diffusion models can effectively remove adv noise
% 3. we theoretically analyze, xxxxx (2 conclusions) (intuition: the union of xxxx, better than rs under general cases)
% 4. in practice, we propose to leverage the majority vote to approximate such high density region and therefore improve the certified robustness
% 5. exp results .....

% \weili{Should we emphasize more the certified robustness in the intro?}

Diffusion models have demonstrated powerful image generation ability recently \citep{Ho2020DDPM, Song2021ICLR} due to the iterative diffusion and denoising processes. Such models so far have achieved the state-of-art performance on sample quality \citep{dhariwal2021diffusion, vahdat2021score}, as well as effective mode coverage \citep{song2021maximum}. 
In particular, diffusion models usually consist of two processes: (i) a forward diffusion process that converts data to noise by gradually adding noise to the input, and (ii) a reverse generative process that starts from noise and generates data by denoising one step at a time~\citep{Song2021ICLR}. 

Given the natural denoising property of diffusion models, \emph{empirical} studies have been conducted to show that it is possible to leverage diffusion models to perform adversarial purification~\citep{nie2022diffusion,wu2022guided,carlini2022certified}. For instance, 
\citeauthor{nie2022diffusion} introduced a diffusion model based purification model  \textit{DiffPure}, which first added Gaussian noises to the adversarial sample to obtain a diffused sample (via diffusion process) and then solved a reverse stochastic differential equation (SDE) (via reverse process) to remove the adversarial perturbation to recover a ``clean" sample. They showed that by carefully choosing the amount of Gaussian noises added during the diffusion process, the adversarial perturbations can be removed while preserving the true label semantics. \citet{carlini2022certified} instantiated the randomized smoothing approach with diffusion model to remove added Gaussian noise, so as to provide certified robustness for a clean model. 


% Despite the empirical success of diffusion models in removing adversarial perturbations, the theoretical understanding for such process is still lacking.
Despite the success of diffusion models in removing adversarial perturbations, the theoretical understanding is still lacking.
In this work, we aim to ask: \textit{What are the sufficient conditions under which a diffusion model is able to remove adversarial perturbation?} \textit{Is it possible to further improve the purification performance based on the fundamental properties of diffusion models?}

% In particular, we theoretically prove that under mild conditions, with the diffusion model, an adversarial example will always be recovered back to the corresponding clean sample with high probability, as long as the data density of the clean samples is high enough.


In this work, we proved that with the diffusion model based adversarial purification pipelines~\cite{xxxx}, an adversarial example will always be recovered back to the corresponding clean sample with high probability, as long as the data density of the clean samples is high enough. \bo{do we want to use clean sample or sample with the ground-truth label here?} In particular, we analyze the properties of the highest density point in the conditional distribution generated by the reverse process of the diffusion model given an adversarial sample. In addition, we theoretically characterized the robust region for each true prototype,\bo{prototype? define it since never mentioned before} within which if the adversarial sample locates, the highest density point will always have the same label as the true prototype.\bo{this sentene is not clear, what's ``locates"?} 
This robustness region is actually the union of all convex sub-regions for prototypes with high density and the same label as the true prototype. We believe that this characterization has the potential to provide larger robustness radius for inputs, since it is able to connect different convex robust sub-regions together\zc{refrase: larger to what?}. In addition, the characterization also implies that the size of robustness regions is affected by the relative density and the distance of true prototype to prototypes with different labels. The influence of these two factors is controlled by the timestamp we choose in the reverse process. 

In practice, it is challenging to exactly sample the point of the highest density in practice as it needs an enormous amount of samplings to make a confident estimation of the densities for all points in the sample space. Thus, we propose to leverage the \textit{majority vote} on the classifier's prediction among different reversed samples to approximate the true prediction. We proved that reverse process of the diffusion model will generate samples in the surrounding neighbourhood of the true prototype where it is more likely that the prototypes with the same label as the true prototype have the highest probability and one such prototype takes the highest density. In this case, \textit{majority vote} will output the label of the highest density point. 

The theoretical analysis enables us to design a certifiably robust adversarial purification pipeline \name (Figure~\ref{pipeline}), which incorporates two steps: (i) we first solve the reverse stochastic differential equation (SDE) to obtain a posterior data distribution conditioned on the input adversarial example, and (ii) then we take the point with the highest density in the obtained distribution as the clean sample, approximated by taking the majority vote for the prediction on different reversed samples.

% In the literature, people are interested in the certified robustness radius, which can be obtained by finding the maximum inclined ball in the robustness region. However, this requires solving an infinite optimization problem due to the infinite number of constraints we use to form the robustness region. Without any restriction on the data distribution, we cannot obtain a certified robustness radius within finite time. Therefore, we resort to the randomized smoothing algorithm~\citep{Cohen2019ICML} to evaluate the certified robustness in practice.

 We conduct extensive experiments on ImageNet and CIFAR-10 datasets under different settings. We show that \name  achieves the new state-of-the-art \emph{certified} robustness on clean model without tuning any model parameters (off-the-shelf).\chaowei{give numbers later}
% We noted that although we can characterize the robust region for an input, generally it is non-convex with (possible) infinite constraints, which makes it hard to find a deterministic certification method to provide the robustness radius (lower bound) for each true prototype. Therefore, we resort to the randomized certification method in \cite{Cohen2019ICML}. On the other hand, we also noted that highest density point locating in high-dimensional spaces requires a huge amount of sampling, which is impossible in practice because we have to solve a SDE for every sampling. As an alternative, we proposed a label majority voting step to approximate the highest density point locating step.

% \vspace{-0.2in}
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\includegraphics[width=0.5\linewidth]{figures/}
\end{center}
% \vspace{-0.2in}
\caption{Pipeline of \name.}\label{pipeline}
\label{robustfigure}
\end{figure}

% \textbf{\underline{Technical Contributions.}}
% In this paper, we take the first step towards understanding the sufficient conditions of \textit{adversarial purification} with diffusion models.
% We make contributions on both theoretical
% and empirical fronts.
% %%\vspace{-0.5em}
% \begin{itemize}[leftmargin=*]
%     \item We proved that under constrained data density property, an adversarial example can be recovered back to the clean sample with high probability via the reverse process of a diffusion model. 
%     \item By choosing the highest density point in the conditional distribution generated by the reverse process of the diffusion model as the ``clean" sample, we theoretically characterized the robustness region for adversarial samples such that the ``clean" sample has the correct label.
%     \item Based on our analysis and with some compromise due to the computation complexity, we proposed \name in practice, which is a state-of-art adversarial purification pipeline directly leveraging the reverse process of a pre-trained diffusion model and a majority vote step.
%     \item We demonstrated state-of-art performance of \name on xxxx
% \end{itemize}

\textbf{\underline{Technical Contributions.}}
In this paper, we take the first step towards understanding the sufficient conditions of \textit{adversarial purification} with diffusion models.
We make contributions on both theoretical
and empirical fronts.
%%\vspace{-0.5em}
\begin{itemize}[leftmargin=*]
    \item We prove that under constrained data density property, an adversarial example can be recovered back to the original clean sample with high probability via the reverse process of a diffusion model.
    \item Based on our analysis, we proposed \name, which is a state-of-art adversarial purification pipeline directly leveraging the reverse process of a pre-trained diffusion model and a highest density point locating step.
    \item We characterized the robust region for each point under \name.
    \item We demonstrated state-of-art performance of \name on xxxx
\end{itemize}


==> sections/intro2_bak2.0.tex <==


\section{Introduction}
% 1. diffusion model is good at removing adv noise based on observations
% 2. but it is unclear about the fundamental reason or sufficient conditions under which diffusion models can effectively remove adv noise
% 3. we theoretically analyze, xxxxx (2 conclusions) (intuition: the union of xxxx, better than rs under general cases)
% 4. in practice, we propose to leverage the majority vote to approximate such high density region and therefore improve the certified robustness
% 5. exp results .....

% \weili{Should we emphasize more the certified robustness in the intro?}

Diffusion models have demonstrated powerful image generation ability recently \citep{Ho2020DDPM, Song2021ICLR} due to the iterative diffusion and denoising processes. Such models so far have achieved state-of-art performance on sample quality \citep{dhariwal2021diffusion, vahdat2021score}, as well as effective mode coverage \citep{song2021maximum}. 
In particular, diffusion models usually consist of two processes: (i) a forward diffusion process that converts data to noise by gradually adding noise to the input, and (ii) a reverse generative process that starts from noise and generates data by denoising one step at a time~\citep{Song2021ICLR}. 

Given the natural denoising property of diffusion models, {empirical} studies have been conducted to show that it is possible to leverage diffusion models to perform adversarial purification~\citep{nie2022diffusion,wu2022guided,carlini2022certified}. For instance, 
\citeauthor{nie2022diffusion} introduced a diffusion model based purification model  \textit{DiffPure}, which first added Gaussian noises to the adversarial sample to obtain a diffused sample (via diffusion process) and then solved a reverse stochastic differential equation (SDE) (via reverse process) to remove the adversarial perturbation to recover a ``clean" sample. They showed that by carefully choosing the amount of Gaussian noises added during the diffusion process, the adversarial perturbations can be removed while preserving the true label semantics. \citet{carlini2022certified} instantiated the randomized smoothing approach with the diffusion model to remove added Gaussian noise, so as to provide certified robustness for a clean model. 


% Despite the empirical success of diffusion models in removing adversarial perturbations, the theoretical understanding for such process is still lacking.
Despite the success of diffusion models in removing adversarial perturbations, theoretical understanding is still lacking. Thus, natural questions emerge: \textit{What are the sufficient conditions under which a diffusion model is able to remove adversarial perturbation?} \textit{Is it possible to further improve the purification performance based on the fundamental properties of diffusion models?}

% In this work, we achieve two goals: (1) we theoretically prove that with the diffusion model based adversarial purification pipelines~\citep{nie2022diffusion}, an adversarial example will always be recovered back to the sample with the ground-truth label with high probability, as long as the data density of the sample with the ground-truth label is high enough; and (2) Based on the theoretical analysis, we propose an effective pipeline, \namens, for adversarial robustness.

% In this work, we theoretically prove that with the diffusion model based adversarial purification pipelines~\citep{nie2022diffusion}, an adversarial example will always be recovered back to the sample with the ground-truth label with high probability, as long as the data density of the sample with the ground-truth label is high enough. Based on the theoretical analysis, we propose an effective pipeline, \name, to improve adversarial robustness compared to \citep{nie2022diffusion}, which incorporates two-step : (i) we first use the reverse process to obtain a posterior data distribution conditioned on the input adversarial example, and (ii) then we take the point with the highest density in the obtained distribution as the clean sample, approximated by taking the majority vote for the prediction on different reversed samples in practical.   


% \bo{do we want to use clean sample or sample with the ground-truth label here?}

In this work, we first prove that given a diffusion model, an adversarial example will always be recovered back to the sample with the ground-truth label with high probability, as long as the data density of the sample with the ground-truth label is high enough. 
% Based on the theoretical analysis, we propose an effective pipeline, \name, to improve adversarial robustness compared to \citep{nie2022diffusion}, which incorporates two-step : (i) we first use the reverse process to obtain a posterior data distribution conditioned on the input adversarial example, and (ii) then we take the point with the highest density in the obtained distribution as the clean sample, approximated by taking the majority vote for the prediction on different reversed samples in practical.   
Concretely, 
% we call the samples in the data manifold as prototypes, which are used to train the classifier. An adversarial sample adds perturbation to a prototype, so that it locates outside of the manifold and mislead the classifier. We call the label corresponding to the attacked prototype as the ground-truth label, and prototypes with the ground-truth label as true prototypes. 
we show that the reverse process of the diffusion model generates a conditional distribution conditioned on a given adversarial sample. We then explicitly characterized the conditional density function whose formulation implies that if the ground-truth samples are of high density, the recovered instance will always be mapped to . 
% On the other hand, these prototypes can be recognized well by classifiers train on the data manifold.

% We show that prototypes near the adversarial sample not only have high density in the conditional distribution, but also keep the label semantics of the adversarial sample. \kj{This sentence needs more reasoning} In other words, the reverse process will highly likely to sample a true prototype. 


For further theoretical analysis, we use the highest density point in the conditional distribution as the clean sample, 
who will be sent to the classifier to predict the ground-truth label. The clean sample will locate in the data manifold and thus the classification outcome will be much more reliable than directly classifying the adversarial sample. 
In addition to the robustness radius studied in previous works, we characterize the robustness region of any true prototype such that all adversarial samples will be classified correctly. We show the robustness region is a union of convex sets, each surrounding a true prototype, and this characterization (the connection of convex sets) has the potential to provide a larger robustness radius than other certification methods \zc{cite} only focusing on the neighborhood of one true prototype. Moreover, the characterization also implies that the size of robustness regions is affected by the relative density and the distance of true prototypes to other prototypes. The influence of these two factors is controlled by the timestamp we choose in the reverse process. 

% In this work, we theoretically characterize the robustness region for a sample with the ground-truth label such that if the adversarial sample lies within the robustness region, the highest density point in the conditional distribution will have the ground truth label. We further show that this robustness region is the union of all convex robustness sub-regions surrounding samples with the ground-truth label. We note that previous works \zc{which to cite} typically focus on investigating the robustness radius in the neighborhood of the only sample, similar to the robustness convex sub-region we established. We believe our characterization has the potential to provide a larger \kj{needs a comparison target} robustness radius compared to the previous work, since it is able to connect different convex robustness sub-regions together\zc{graph}. In addition, the characterization also implies that the size of robustness regions is affected by the relative density and the distance of true prototype \kj{this is the first time we see the term ``prototype'', and we should give it a definition or say it's equivalent to a clean sample with ground truth label} to prototypes with different labels. The influence of these two factors is controlled by the timestamp we choose in the reverse process. 

% \kj{Not the best way to say it, but probably a way to reduce the repetitiveness in some sentences.\\
% In addition to the robustness radius studied in previous works, we characterize the robustness region of a sample with a ground truth label such that all adversarial samples within will be classified with the ground truth label. We further show the robustness region is a union of convex sets, each surrounding a sample with the same ground truth label as the current sample, and this characterization (the connection of convex sets) has the potential to provide a large robustness radius.}


Based on the above analysis, we design \name as shown in Figure~\ref{}, consisting of two steps: (i) we first use the reverse process of diffusion model to obtain a posterior data distribution conditioned on the input adversarial example; and (ii) we perform the reverse process multiple times to approximate the high density instances via majority vote. 
We conduct extensive experiments on ImageNet and CIFAR-10 datasets under different settings to evaluate the certifiable robustness of \name. In particular, we follow the setting from \citet{carlini2022certified} and rely on  randomized smoothing to certify robustness to adversarial perturbations bounded in the $\mathcal{L}_2$-norm.   We show that \name~ achieves the new state-of-the-art \emph{certified} robustness on the clean model without tuning any model parameters (off-the-shelf). \name obtains significantly better certified robustness results  xxxx
% The second step is hard to implement in practice as it needs an enormous amount of samplings to make a confident estimation of the densities 
% for all points 
% in the sample space. Thus, in practice, we feed the input adversarial example multiple time into the reverse process and leverage the \textit{majority vote} on the classifier's prediction among different reversed samples to approximate the true prediction. 
% We prove that the reverse process of the diffusion model will generate samples in the surrounding neighborhood of the true prototypes with high probability. This implies that  \textit{majority vote} will high likely output the label of the highest density point, which is also the ground-truth label.


% \kj{Should we flip the order of this and the next paragraph?}




% approximated by taking the majority vote for the prediction on different reversed samples in practice. 

%%%%%%%
%%%%%%%
%%%%%%%
%%%%%%%
% In practice, it is challenging to exactly sample the point of the highest density in practice as it needs an enormous amount of samplings to make a confident estimation of the densities for all points in the sample space. Thus, we propose to leverage the \textit{majority vote} on the classifier's prediction among different reversed samples to approximate the true prediction. We proved that the reverse process of the diffusion model will generate samples in the surrounding neighborhood of the true prototype where it is more likely that the prototypes with the same label as the true prototype have the highest probability and one such prototype takes the highest density. In this case, \textit{majority vote} will output the label of the highest density point. \kj{Should we flip the order of this and the next paragraph?}

% The above analysis enables us to design a certifiably robust adversarial purification pipeline \name~ (Figure~\ref{pipeline}), which incorporates two steps: (i) we first solve the reverse stochastic differential equation (SDE) to obtain a posterior data distribution conditioned on the input adversarial example, and (ii) then we take the point with the highest density in the obtained distribution as the clean sample, approximated by taking the majority vote for the prediction on different reversed samples.
%%%%%%%
%%%%%%%
%%%%%%%
%%%%%%%

% In the literature, people are interested in the certified robustness radius, which can be obtained by finding the maximum inclined ball in the robustness region. However, this requires solving an infinite optimization problem due to the infinite number of constraints we use to form the robustness region. Without any restriction on the data distribution, we cannot obtain a certified robustness radius within finite time. Therefore, we resort to the randomized smoothing algorithm~\citep{Cohen2019ICML} to evaluate the certified robustness in practice.


% We noted that although we can characterize the robust region for an input, generally it is non-convex with (possible) infinite constraints, which makes it hard to find a deterministic certification method to provide the robustness radius (lower bound) for each true prototype. Therefore, we resort to the randomized certification method in \cite{Cohen2019ICML}. On the other hand, we also noted that highest density point locating in high-dimensional spaces requires a huge amount of sampling, which is impossible in practice because we have to solve a SDE for every sampling. As an alternative, we proposed a label majority voting step to approximate the highest density point locating step.

% \vspace{-0.2in}
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\includegraphics[width=0.5\linewidth]{figures/}
\end{center}
% \vspace{-0.2in}
\caption{Pipeline of \name.}\label{pipeline}
\label{robustfigure}
\end{figure}

% \textbf{\underline{Technical Contributions.}}
% In this paper, we take the first step towards understanding the sufficient conditions of \textit{adversarial purification} with diffusion models.
% We make contributions on both theoretical
% and empirical fronts.
% %%\vspace{-0.5em}
% \begin{itemize}[leftmargin=*]
%     \item We proved that under constrained data density property, an adversarial example can be recovered back to the clean sample with high probability via the reverse process of a diffusion model. 
%     \item By choosing the highest density point in the conditional distribution generated by the reverse process of the diffusion model as the ``clean" sample, we theoretically characterized the robustness region for adversarial samples such that the ``clean" sample has the correct label.
%     \item Based on our analysis and with some compromise due to the computation complexity, we proposed \name in practice, which is a state-of-art adversarial purification pipeline directly leveraging the reverse process of a pre-trained diffusion model and a majority vote step.
%     \item We demonstrated state-of-art performance of \name on xxxx
% \end{itemize}

\textbf{\underline{Technical Contributions.}}
In this paper, we take the first step towards understanding the sufficient conditions of \textit{adversarial purification} with diffusion models.
We make contributions on both theoretical
and empirical fronts.
%%\vspace{-0.5em}
\begin{itemize}[leftmargin=*]
    \item We prove that under constrained data density property, an adversarial example can be recovered back to the original clean sample with high probability via the reverse process of a diffusion model.
    \item Based on our analysis, we proposed \name, which is a state-of-art adversarial purification pipeline directly leveraging the reverse process of a pre-trained diffusion model and a highest density point locating step.
    \item We characterized the robust region for each point under \name.
    \item We demonstrated state-of-art performance of \name~ on xxxx
\end{itemize}


==> sections/intro_v3.tex <==


\section{Introduction}
% 1. diffusion model is good at removing adv noise based on observations
% 2. but it is unclear about the fundamental reason or sufficient conditions under which diffusion models can effectively remove adv noise
% 3. we theoretically analyze, xxxxx (2 conclusions) (intuition: the union of xxxx, better than rs under general cases)
% 4. in practice, we propose to leverage the majority vote to approximate such high density region and therefore improve the certified robustness
% 5. exp results .....

% \weili{Should we emphasize more the certified robustness in the intro?}

Diffusion models have demonstrated powerful image generation ability recently \citep{Ho2020DDPM, Song2021ICLR} due to the iterative diffusion and denoising processes. Such models so far have achieved state-of-the-art performance on sample quality \citep{dhariwal2021diffusion, vahdat2021score}, as well as effective mode coverage \citep{song2021maximum}. 
Diffusion models usually consist of two processes: (i) a forward diffusion process that converts data to noise by gradually adding noise to the input, and (ii) a reverse generative process that starts from noise and generates data by denoising one step at a time~\citep{Song2021ICLR}. 

Given the natural denoising property of diffusion models, \emph{empirical} studies have leveraged them to perform adversarial purification~\citep{nie2022diffusion,wu2022guided,carlini2022certified}. For instance, 
\citeauthor{nie2022diffusion} introduced a diffusion model based purification model  \textit{DiffPure}.
% , which first adds Gaussian noises to the adversarial sample to obtain a diffused sample (via diffusion process), and then solves a reverse stochastic differential equation (SDE) (via reverse process) to remove the adversarial perturbation to recover a ``clean" sample. 
They showed that by carefully choosing the amount of Gaussian noises added during the diffusion process, the adversarial perturbations can be removed while preserving the true label semantics {\em empirically}. 
\citet{carlini2022certified} instantiated the randomized smoothing approach with the diffusion model to remove added Gaussian noise. They viewed the diffusion model as a {\em blackbox} and showed that using a diffusion model achieves nontrivial certified robustness, which offers a {\em provable guarantee} that a clean model's prediction is robust to  $L_2$-norm bounded adversarial example.
% so as to provide certified robustness which offers a provable guarantee that a clean model's prediction is robust to  $L_2$-norm bounded adversarial example.


% Despite the empirical success of diffusion models in removing adversarial perturbations, the theoretical understanding for such process is still lacking.
Despite the success of diffusion models in removing adversarial perturbations, theoretical understanding is still lacking. Thus, natural questions emerge: \textit{What are the sufficient conditions under which a diffusion model is able to remove adversarial perturbation?} \textit{Is it possible to further improve the purification performance (e.g., certified robustness) based on the fundamental properties of diffusion models?}

In this work,  we prove that given a diffusion model, an adversarial example will  be recovered back to the sample with the ground-truth label with high probability, as long as the \textit{data} density of the samples with the ground-truth label is high enough. 
% Based on our theoretical analysis, we propose an effective pipeline, \name.
% we achieve two goals: (1) we theoretically prove that with the diffusion model based adversarial purification pipelines~\citep{nie2022diffusion}, an adversarial example will always be recovered back to the sample with the ground-truth label with high probability, as long as the data density of the sample with the ground-truth label is high enough; and (2) Based on the theoretical analysis, 
% In this work, we theoretically prove that with the diffusion model based adversarial purification pipelines~\citep{nie2022diffusion}, an adversarial example will always be recovered back to the sample with the ground-truth label with high probability, as long as the data density of the sample with the ground-truth label is high enough. Based on the theoretical analysis, we propose an effective pipeline, \name, to improve adversarial robustness compared to \citep{nie2022diffusion}, which incorporates two-step : (i) we first use the reverse process to obtain a posterior data distribution conditioned on the input adversarial example, and (ii) then we take the point with the highest density in the obtained distribution as the clean sample, approximated by taking the majority vote for the prediction on different reversed samples in practical.   
% \bo{do we want to use clean sample or sample with the ground-truth label here?}
Concretely, when we directly feed an adversarial example into the reverse process of a diffusion model, the reverse process generates a distribution over the training data manifold conditioned on the given adversarial sample. We explicitly characterize the  obtained conditional density function, and show that as long as the data manifold with the ground-truth label has a higher conditional density than the manifolds with other labels, the reversed sample will have a high probability to be mapped to the manifold with ground-truth prediction. 
% Thus, If we use the highest density point in the conditional distribution as the reversed sample, it is more likely to predict the reversed sample as ground-truth compared to directly feeding the adversarial examples into the classifier. 
% Moreover, if the density of the ground-truth label is high enough, the reversed example will always be predicted as the ground-truth label.  



For further theoretical analysis,  we take the highest density point in the conditional distribution as the reversed sample for the classifier prediction. We identify that the robust region for a given instance under the diffusion model reverse process is the union of multiple convex sets, each surrounding a manifold with the ground-truth label. 
% we study the robustness radius of the above process.
% We characterize the robustness region of any true prototype such that all adversarial samples will be classified correctly.
% We characterize the robustness region of any data manifolds with the ground-truth label such that all adversarial samples will be classified correctly.
% we characterize the robustness region of adversarial samples which will be classified correctly.
% We show that such robust region is a union of multiple convex sets, each surrounding a manifold with the ground-truth label. 
Compared with the robustness region of previous work~\cite{Cohen2019ICML}, which only focuses on the neighborhood of {\em one} manifold with the ground-truth label, such union of multiple convex sets has the potential to provide a much larger robust region. 
Moreover, the characterization implies that the size of robust regions is affected by the relative density and the distance between data manifolds with the ground-truth label and those with other labels. 
% The influence of these two factors is controlled by the timestamp we choose in the reverse process.  \chaowei{Not sure whether we need the last two sentences. I find it not strictly connected with the previous sentences. It seems that we miss something in the middle. }
% The influence of these two factors is controlled by the timestamp we choose in the reverse process. 



In practice, inspired by our theoretical analysis, we propose a pipeline \namens, which incorporates two steps:  (i) using the reverse process of the diffusion model to obtain a sample of the posterior data distribution conditioned on the adversarial input; and (ii)  repeating the reverse process multiple times to approximate the label of high density manifold via majority vote. 
In particular,  given an adversarial input, we repeatedly feed it into the reverse process of the diffusion model to get multiple reversed examples and feed them into the classifier to get the final prediction. We then apply the \textit{majority vote} on such predictions to get the final predicted label.

We conduct extensive experiments on ImageNet and CIFAR-10 datasets under different settings to evaluate the certifiable robustness of \namens. In particular, we follow the setting from \citet{carlini2022certified} and rely on  randomized smoothing to certify robustness to adversarial perturbations bounded in the $\mathcal{L}_2$-norm.   We show that \name achieves the new state-of-the-art \emph{certified} robustness on the clean model without tuning any model parameters (off-the-shelf). 
% \name obtains significantly better certified robustness results. 
On ImageNet, it achieves a consistently higher certified accuracy than the existing methods among every $\sigma$ at every radius $\epsilon$ , 7\% improvement on average.     
% We noted that although we can characterize the robust region for an input, generally it is non-convex with (possible) infinite constraints, which makes it hard to find a deterministic certification method to provide the robustness radius (lower bound) for each true prototype. Therefore, we resort to the randomized certification method in \cite{Cohen2019ICML}. On the other hand, we also noted that highest density point locating in high-dimensional spaces requires a huge amount of sampling, which is impossible in practice because we have to solve a SDE for every sampling. As an alternative, we proposed a label majority voting step to approximate the highest density point locating step.

% \vspace{-0.2in}
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\includegraphics[width=0.75\linewidth]{figures/densepure_flowchart.png}
\end{center}
% \vspace{-0.2in}
\caption{Pipeline of \namens.}\label{pipeline}
\label{robustfigure}
\end{figure}

% \textbf{\underline{Technical Contributions.}}
% In this paper, we take the first step towards understanding the sufficient conditions of \textit{adversarial purification} with diffusion models.
% We make contributions on both theoretical
% and empirical fronts.
% %%\vspace{-0.5em}
% \begin{itemize}[leftmargin=*]
%     \item We proved that under constrained data density property, an adversarial example can be recovered back to the clean sample with high probability via the reverse process of a diffusion model. 
%     \item By choosing the highest density point in the conditional distribution generated by the reverse process of the diffusion model as the ``clean" sample, we theoretically characterized the robustness region for adversarial samples such that the ``clean" sample has the correct label.
%     \item Based on our analysis and with some compromise due to the computation complexity, we proposed \name in practice, which is a state-of-art adversarial purification pipeline directly leveraging the reverse process of a pre-trained diffusion model and a majority vote step.
%     \item We demonstrated state-of-art performance of \name on xxxx
% \end{itemize}

\textbf{\underline{Technical Contributions.}}
In this paper, we take the first step towards understanding the sufficient conditions of \textit{adversarial purification} with diffusion models.
We make contributions on both theoretical
and empirical fronts: (1) We prove that under constrained data density property, an adversarial example can be recovered back to the original clean sample with high probability via the reverse process of a diffusion model.
    (2) In theory, we characterized the robust region for each point by further taking the highest density point in the conditional distribution generated by the reverse process as the reversed sample. 
    (3) In practice, we proposed \namens, which is a state-of-art adversarial purification pipeline directly leveraging the reverse process of a pre-trained diffusion model and label \textit{majority vote}.
    (4) We demonstrated state-of-art performance of \name on ImageNet and CIFAR-10.

%%\vspace{-0.5em}
% \begin{itemize}[leftmargin=*]
%     \item We prove that under constrained data density property, an adversarial example can be recovered back to the original clean sample with high probability via the reverse process of a diffusion model.
%     \item In theory, we characterized the robust region for each point by further taking the highest density point in the conditional distribution generated by the reverse process as the reversed sample. 
%     \item In practice, we proposed \namens, which is a state-of-art adversarial purification pipeline directly leveraging the reverse process of a pre-trained diffusion model and label \textit{majority vote}.
%     \item We demonstrated state-of-art performance of \name on xxxx \zc{fill in}
% \end{itemize}

% \begin{figure}[h]
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \includegraphics[width=0.85\linewidth]{figures/densepure_robustness_region.png}
% \end{center}
% % \vspace{-0.2in}
% \caption{Base classifier vs \namens.}\label{pipeline}
% \label{robustfigure}
% \end{figure}

==> sections/intro_v4.tex <==


\section{Introduction}
% 1. diffusion model is good at removing adv noise based on observations
% 2. but it is unclear about the fundamental reason or sufficient conditions under which diffusion models can effectively remove adv noise
% 3. we theoretically analyze, xxxxx (2 conclusions) (intuition: the union of xxxx, better than rs under general cases)
% 4. in practice, we propose to leverage the majority vote to approximate such high density region and therefore improve the certified robustness
% 5. exp results .....

% \weili{Should we emphasize more the certified robustness in the intro?}

Diffusion models have been shown to be a powerful image generation tool \citep{Ho2020DDPM, Song2021ICLR} owing to their iterative diffusion and denoising processes. These models have achieved state-of-the-art performance on sample quality \citep{dhariwal2021diffusion, vahdat2021score} as well as effective mode coverage \citep{song2021maximum}. 
A diffusion model usually consists of two processes: (i) a forward diffusion process that converts data to noise by gradually adding noise to the input, and (ii) a reverse generative process that starts from noise and generates data by denoising one step at a time~\citep{Song2021ICLR}. 

Given the natural denoising property of diffusion models, \emph{empirical} studies have leveraged them to perform adversarial purification~\citep{nie2022diffusion,wu2022guided,carlini2022certified}. For instance, 
\citeauthor{nie2022diffusion} introduce a diffusion model based purification model  \textit{DiffPure}. 
% , which first adds Gaussian noises to the adversarial sample to obtain a diffused sample (via diffusion process), and then solves a reverse stochastic differential equation (SDE) (via reverse process) to remove the adversarial perturbation to recover a ``clean" sample. 
They {\em empirically} show that by carefully choosing the amount of Gaussian noises added during the diffusion process, adversarial perturbations can be removed while preserving the true label semantics. 
Despite the significant empirical results, there is no provable guarantee on the robustness. 
\citet{carlini2022certified} instantiate the randomized smoothing approach with the diffusion model to offer a {\em provable guarantee}  of model robustness against   $L_2$-norm bounded adversarial example.
% that  model's prediction is robust to  $L_2$-norm bounded adversarial example.
% However, they view the diffusion model as a {\em blackbox} without having a theoretical understanding of why and how the diffusion models contribute to  such nontrivial  certified robustness. 
However, they do not provide a theoretical understanding of why and how the diffusion models contribute to  such nontrivial  certified robustness. 
% so as to provide certified robustness which offers a provable guarantee that a clean model's prediction is robust to  $L_2$-norm bounded adversarial example.
% Despite the empirical success of diffusion models in removing adversarial perturbations, the theoretical understanding for such process is still lacking.
% Despite the success of diffusion models for adversarial robustness, theoretical understanding is still lacking. 
% Thus,  natural questions emerge: \textit{What are the sufficient conditions under which a diffusion model is able to remove adversarial perturbation?} \textit{Is it possible to further improve the purification performance (i.e., certified robustness) based on the fundamental properties of diffusion models?}

\textbf{Our Approach.} We theoretically analyze the fundamental properties of diffusion models to understand why and how it enhances certified robustness, which then allows us to propose \namens, which improves the certified robustness of a given model by more effectively using the diffusion  model.


% \textbf{Our Approach.} We analyze theoretically the fundamental properties of diffusion model in why and how it can enhance certified robustness. 
% Based on these properties, we propose densepure propose \name to improve the certified robustness of a standard model by properly using the diffusion  model.

We theoretically prove that given a diffusion model, an adversarial example can be corrected back to the sample with the ground-truth label with high probability, as long as the \textit{data} density of the samples with the ground-truth label is sufficiently high. 
% Based on our theoretical analysis, we propose an effective pipeline, \name.
% we achieve two goals: (1) we theoretically prove that with the diffusion model based adversarial purification pipelines~\citep{nie2022diffusion}, an adversarial example will always be recovered back to the sample with the ground-truth label with high probability, as long as the data density of the sample with the ground-truth label is high enough; and (2) Based on the theoretical analysis, 
% In this work, we theoretically prove that with the diffusion model based adversarial purification pipelines~\citep{nie2022diffusion}, an adversarial example will always be recovered back to the sample with the ground-truth label with high probability, as long as the data density of the sample with the ground-truth label is high enough. Based on the theoretical analysis, we propose an effective pipeline, \name, to improve adversarial robustness compared to \citep{nie2022diffusion}, which incorporates two-step : (i) we first use the reverse process to obtain a posterior data distribution conditioned on the input adversarial example, and (ii) then we take the point with the highest density in the obtained distribution as the clean sample, approximated by taking the majority vote for the prediction on different reversed samples in practical.   
% \bo{do we want to use clean sample or sample with the ground-truth label here?}
Concretely, when we directly feed an adversarial example into the reverse process of a diffusion model, the reverse process generates a distribution over the training data region conditioned on the given adversarial sample. We explicitly characterize the  obtained conditional density function, and show that as long as the data region with the ground-truth label has a higher 
% conditional\zc{should be data density instead of conditional density} 
data density than the regions with other labels, the reversed sample will have a high probability to be mapped to the region with ground-truth prediction. 
% Thus, If we use the highest density point in the conditional distribution as the reversed sample, it is more likely to predict the reversed sample as ground-truth compared to directly feeding the adversarial examples into the classifier. 
% Moreover, if the density of the ground-truth label is high enough, the reversed example will always be predicted as the ground-truth label.  



 We then use the highest density point in the conditional distribution as the denoised sample for the classifier prediction. 
We show that the robust region for a given sample under the diffusion model's reverse process is the union of multiple convex sets, each surrounding a region around the ground-truth label. 
% we study the robustness radius of the above process.
% We characterize the robustness region of any true prototype such that all adversarial samples will be classified correctly.
% We characterize the robustness region of any data regions with the ground-truth label such that all adversarial samples will be classified correctly.
% we characterize the robustness region of adversarial samples which will be classified correctly.
% We show that such robust region is a union of multiple convex sets, each surrounding a region with the ground-truth label. 
Compared with the robust region identified in previous work~\citep{Cohen2019ICML}, which only focuses on the neighborhood of {\em one} region with the ground-truth label, such union of multiple convex sets can provide a much larger robust region. 
Moreover, the characterization implies that the size of robust regions is affected by the relative density and the distance between data regions with the ground-truth label and those with other labels. 
% The influence of these two factors is controlled by the timestamp we choose in the reverse process.  \chaowei{Not sure whether we need the last two sentences. I find it not strictly connected with the previous sentences. It seems that we miss something in the middle. }
% The influence of these two factors is controlled by the timestamp we choose in the reverse process. 



In practice, \name is designed to approximate the label of the high density region in the conditional distribution by incorporating two steps: (i) using the reverse process of the diffusion model to obtain a sample of the posterior data distribution conditioned on the adversarial input; and (ii)  
repeating the reverse process multiple times to approximate the label of high density region in the conditional distribution via a  majority vote. 
In particular,  given an adversarial input, we repeatedly feed it into the reverse process of the diffusion model to get multiple reversed examples and feed them into the classifier to get the final prediction. We then apply the \textit{majority vote} on such predictions to get the final predicted label.

We conduct extensive experiments on ImageNet and CIFAR-10 datasets under different settings to evaluate the certifiable robustness of \namens. In particular, we follow the setting from \citet{carlini2022certified} and rely on  randomized smoothing to certify robustness to adversarial perturbations bounded in the $\mathcal{L}_2$-norm.   We show that \name achieves the new state-of-the-art \emph{certified} robustness on the clean model without tuning any model parameters (off-the-shelf). 
% \name obtains significantly better certified robustness results. 
On ImageNet, it achieves a consistently higher certified accuracy than the existing methods among every $\sigma$ at every radius $\epsilon$ , 7\% improvement on average.     
% We noted that although we can characterize the robust region for an input, generally it is non-convex with (possible) infinite constraints, which makes it hard to find a deterministic certification method to provide the robustness radius (lower bound) for each true prototype. Therefore, we resort to the randomized certification method in \cite{Cohen2019ICML}. On the other hand, we also noted that highest density point locating in high-dimensional spaces requires a huge amount of sampling, which is impossible in practice because we have to solve a SDE for every sampling. As an alternative, we proposed a label majority voting step to approximate the highest density point locating step.

% \vspace{-0.2in}
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\includegraphics[width=0.75\linewidth]{figures/densepure_flowchart.png}
\end{center}
% \vspace{-0.2in}
\caption{Pipeline of \namens.}\label{pipeline}
\label{robustfigure}
\end{figure}

% \textbf{\underline{Technical Contributions.}}
% In this paper, we take the first step towards understanding the sufficient conditions of \textit{adversarial purification} with diffusion models.
% We make contributions on both theoretical
% and empirical fronts.
% %%\vspace{-0.5em}
% \begin{itemize}[leftmargin=*]
%     \item We proved that under constrained data density property, an adversarial example can be recovered back to the clean sample with high probability via the reverse process of a diffusion model. 
%     \item By choosing the highest density point in the conditional distribution generated by the reverse process of the diffusion model as the ``clean" sample, we theoretically characterized the robustness region for adversarial samples such that the ``clean" sample has the correct label.
%     \item Based on our analysis and with some compromise due to the computation complexity, we proposed \name in practice, which is a state-of-art adversarial purification pipeline directly leveraging the reverse process of a pre-trained diffusion model and a majority vote step.
%     \item We demonstrated state-of-art performance of \name on xxxx
% \end{itemize}

\textbf{\underline{Technical Contributions.}}
In this paper, we take the first step towards understanding the sufficient conditions of \textit{adversarial purification} with diffusion models.
We make contributions on both theoretical
and empirical fronts: (1) We prove that under constrained data density property, an adversarial example can be recovered back to the original clean sample with high probability via the reverse process of a diffusion model.
    (2) In theory, we characterize the robust region for each point by further taking the highest density point in the conditional distribution generated by the reverse process as the reversed sample. 
    (3) In practice, we propose \namens, which is a state-of-art adversarial purification pipeline directly leveraging the reverse process of a pre-trained diffusion model and label \textit{majority vote}.
    (4) We demonstrate state-of-the-art performance of \name on ImageNet and CIFAR-10.

%%\vspace{-0.5em}
% \begin{itemize}[leftmargin=*]
%     \item We prove that under constrained data density property, an adversarial example can be recovered back to the original clean sample with high probability via the reverse process of a diffusion model.
%     \item In theory, we characterized the robust region for each point by further taking the highest density point in the conditional distribution generated by the reverse process as the reversed sample. 
%     \item In practice, we proposed \namens, which is a state-of-art adversarial purification pipeline directly leveraging the reverse process of a pre-trained diffusion model and label \textit{majority vote}.
%     \item We demonstrated state-of-art performance of \name on xxxx \zc{fill in}
% \end{itemize}

% \begin{figure}[h]
% \begin{center}
% %\framebox[4.0in]{$\;$}
% \includegraphics[width=0.85\linewidth]{figures/densepure_robustness_region.png}
% \end{center}
% % \vspace{-0.2in}
% \caption{Base classifier vs \namens.}\label{pipeline}
% \label{robustfigure}
% \end{figure}

==> sections/method_bak.tex <==
\section{\name }
Based on the theoretical analysis introduced before, it inspires us to propose the robust framework, \name. In this section, we will introduce \name and show how to calculate the  certified robustness via randomized smoothing algorithm. 
% Since it is hard to find the density region, here we empirically leverage the majority vote to estimate it.  
\paragraph{Framework. }
Our framework, \name,  consists of two components: (1)  an off-the-self diffusion model and (2) a classifier trained on the standard clean dataset (e.g. ImageNet).
Given an adversarial input, \name incorporates two steps for adversarial robustness. First, we feed the adversarial input into  the reverse process of the diffusion model to obtain a posterior data distribution conditioned on the input adversarial example. Second, we take the point with the highest density in the obtained distribution as the purified sample.  Note that  as we have shown before, diffusion process itself is not necessary when leveraging diffusion models for adversarial purification. Instead, by sending the adversarial example directly through the reverse process of the diffusion model, we can obtain a better-recovered sample in terms of its distance to the corresponding clean sample. Thus, \name indeed removes the diffusion process of the diffusion model in our pipeline. 



% Note that here, we do remove the diffusion process of the diffusion model, instead,  by sending the adversarial example directly through the reverse process of the diffusion model. Our following theorem shows that we can obtain a better-recovered sample in terms of its distance to the corresponding clean sample
% \chaowei{Give a proof.}



When applying the above steps in practice, One challenge is that find the point with the highest density in the obtained distribution since it requires an enormous amount of samplings to confidently estimate the densities in the whole sample space.  For diffusion model, it is already quite expensive to even do sampling once. Thus, it is almost impossible to find such the point. 
% Because we need a huge amount of
% samplings to makes a confidential estimation of the densities for all points in the sample space. For
% diffusion model, it is quite expensive to even do sampling once.
To address it,  we approximate  the second step with \textit{majority vote} to reduce the heavy computation. Specifically,  if we only focus on classification, we first repeatedly send the scaled perturbed sample $\dst \vx_{a,t}$ through the reverse process of the diffusion to obtain multiple reversed samples and feed them into the classifier
to get the predictions. Then we use the majority vote on such predictions to provide the final label assigned to $\dst \vx_a$. When most of the samples surround the true sample $\dst \vx_0$, we can say the label majority vote will give the label of the highest density point with high probability. \chaowei{@zhongzhu}

\paragraph{Certified Robustness with \name}
% First, similar to \citet{carlini2022certified}, our framework first map the randomized smoothing noise $\sigma$ to the noise used for the forward process of the diffusion model. Specifically, given a randomized smoothing parameter $\sigma$ and data input example $x$, randomized smoothing adds a Gaussian noise $\epsilon$, where $\epsilon \sim \mathcal{N}(0, \sigma^2 I)$ to $x$. We could directly map randomized example $x_{\text{rs}} = x+\epsilon$ with the forward processing of the diffusion model $x_\text{rs} = x_t \sim \mathcal{N}(\sqrt{\alpha_t} x_0, (1-\alpha_t) I) $  as :   
% \begin{equation*}
%     \sigma^2 = \frac{1-\alpha_t}{\alpha_t}
% \end{equation*}
% In this way, it equals to  calculate the corresponding timestep $t$ to satisfy the above equation. \chaowei{@jiongxiao, transfer it to SDE. }
Here, we show how to use Randomized Smoothing (RS)\citep{Cohen2019ICML} to calculate the certified robustness of \name. We follow the similar process of \citet{carlini2022certified}. Specifically, our framework first calculate the $t$, the step used for reverse process of diffusion model. To calculate it, given a  Gaussian noise $\epsilon \sim N(0, \sigma^2I)$,  randomized smoothing adds $\epsilon$ to data input $x$ to get the randomized data input $x_\text{rs} = x+\epsilon$. Thus, we map the randomized example $x_\text{rs}$ to data $x_t$ with $t$ step diffusion processing, where $x_t \sim \sqrt{\alpha_t}\mathcal{N}(x_0, \frac{1-\alpha_t}{\alpha_t} I)$ so that $\sigma^2 = \frac{1-\alpha_t}{\alpha_t}$.
% $\sqrt{\alpha_t}x_\text{rs}=x_t\sim \mathcal{N}(\sqrt{\alpha_t} x_0, \alpha_t \sigma^2  I)$. Knowing the true distribution of $x_t \sim \mathcal{N}(\sqrt{\alpha_t} x_0, (1-\alpha_t) I)$, 
In this way, we could directly compute $\alpha_t$ as:
% \begin{equation*}
    $\alpha_t = \frac{1}{1+\sigma^2}$
% \end{equation*}
After that, we can get the corresponding t of SDE by solving the following equation based on the selected schedule $\beta(t)$:
\begin{equation*}
    \alpha_t = e^{-\int_0^t\beta(s)ds}
\end{equation*}
For discrete $\beta(t)$ schedule, we choose the timestep t which makes $\sqrt{\alpha_t}$ the nearest value to $\frac{1}{1+\sigma^2}$ in the set $\left\{\sqrt{\alpha_s} | s=1...T \right\}$.


Second, given the timestep $t$, we could feed the randomized smoothing sample $x_{rs}$ into the reverse processing of the diffusion to resample the original input $\hat{x_{0}}$, denoting as $\hat{x_{0}} = \text{Reverse}(x_{rs}, t)$.  As mentioned before, \name needs to locate the highest density point in the conditional distribution $\dst  p\left(\hat{\rvx}_0 =\vx| {\hat {\rvx}_t = \vx_{a,t}}\right)$ characterized by Theorem \ref{distribution:reverse}. However, it is hard to do it in reality since we need a huge amount of samplings to makes a confidential estimation of the densities for all points in the sample space. It is extremely computational expensive in the high dimensional space. Thus, here we propose a simple but efficient strategy: \textit{majority voting}. 

Since the reversed sample will be fed into the classifier for certification,  if we only focus on classification, we propose to replace the highest density point locating step with label majority vote step to reduce the heavy computation. In other words, we first send the randomized sample $x_{rs}$ through the reverse process of the diffusion model $b$ times to obtain $b$ samples of the conditional distribution, then we use the majority label of these samples as the label.  The algorithm has been shown in Algo~\ref{}.


\paragraph{Reduced  reverse sampling steps.}
For the reverse process of the diffusion model, it requires to repeatedly apply a ``single-step'' operation $t$ times to  (e.g. $x_{0} = Denoise( \cdots Denoise( Denoise(x_t; t); t-1); \cdots 1)$). Here $x_{t-1} = Denoise(x_t;t)$ means we sample $x_{t-1} \sim \mathcal{N}(\widetilde{\mu}(x_t,x_0), \widetilde{\beta}_t I)$, where
\begin{equation*}
    \widetilde{\mu}(x_t,x_0) := \frac{\sqrt{\alpha_{t-1}}\beta_t}{1-\alpha_t}x_0 + \frac{\sqrt{\alpha_t}(1-\alpha_{t-1})}{1-\alpha_t}x_t
\end{equation*}

Thus, using single step repeatedly to perform the whole reverse process in the diffusion model is really time-consuming process. Instead of using single step, here we reduce the repeatedly single-step reverse sampling processing to $st$-step  sparse sampling strategy by changing the reverse sampling schedule from $\{t, t-1, \cdots, 1\}$ to $\{t, t-[\frac{t}{st}], \cdots, 1 \}$, where we fix the last step $t-st[\frac{t}{st}]$ to 1, so that   $x_{0} = Denoise( \cdots Denoise( Denoise(x_t; t-[\frac{t}{st}]); t- [\frac{2t}{st}]); \cdots ;1)$. In details, 
% \chaowei{The following needs to be changed! }


For the new reverse sampling schedule $S = \{t, t-[\frac{t}{st}], \cdots, 1 \}$, we need to revise our $\alpha_t$ to make it adapted to our reduced reverse sampling methods. If we denote $S_t$ as the $t\text{th}$ element in $S$, we will have the new noise schedule $\alpha_{S_t}$, which can be used to compute the following $\beta_{S_t}$ and $\widetilde{\beta}_{S_t}$:
\begin{equation*}
  \beta_{S_t} = 1 - \frac{\alpha_{S_t}}{\alpha_{S_{t-1}}},   \quad \widetilde{\beta}_{S_t} = \frac{1-\alpha_{S_{t-1}}}{1-\alpha_{S_t}}\beta_{S_t}
\end{equation*}
Then we can sample $x_{S_{t-1}} \sim \mathcal{N}(\widetilde{\mu}(x_{S_{t}},x_0), \widetilde{\beta}_{S_t} I)$ step by step to speed up sampling in only $st$ steps.
% \begin{equation*}
%     \widetilde{\mu}(x_{S_{t}},x_0) := \frac{\sqrt{\alpha_{S_{t-1}}}\beta_{S_t}}{1-\alpha_{S_t}}x_0 + \frac{\sqrt{\alpha_{S_t}}(1-\alpha_{S_{t-1}})}{1-\alpha_{S_t}}x_{S_t}
% \end{equation*}




% If $st$ is too small,  $st$-step  sparse sampling strategy leads to a bad image quality after the reverse process. Thus, there exists a tradeoff to balance the quality and speed. 
% we finally use 10 steps during sampling. For fast sampling, we used Improving Sampling Speed method in \cite{}. 
% If the total number of sampling is $T$ steps, we can choose an arbitrary subsequence S of $1...T$ and do the reverse process just in t stpes, which is the length of subsequence S. For a give noise schedule $\overline{a}_t$, we can obtain the schedule $\overline{a}_{S_t}$, which is also a subset of $\overline{a}_t$. Then we will obtain sampling variances as
% \begin{equation*}
%   \beta_{S_t} = 1 - \frac{\overline{a}_{S_t}}{\overline{a}_{S_{t-1}}},   \quad \widetilde{\beta}_{S_t} = \frac{1-{S_{t-1}}}{1-{S_t}}\beta_{S_t}
% \end{equation*}
% Using such parameters, we can realize our reduced sampling steps. For the subsequence strategy, we simply do an equally partition to the total $T$ steps.


% We also find that larger sampling steps normally need more majority voting numbers to achieve their best results. This is because larger sampling steps will add more noise during reverse process. But the one step sampling method does not add any noise during reverse, so majority voting is not proper for one step method. 



% By using the majority vote strategy,when most of the samples surround the true sample $\dst \vx_0$, we can say the label majority vote will give the label of the highest density point with high probability. The following theorem is an adaptation of \cite[Theorem 3.2]{nie2022diffusion} bounding the distance of the samples in $\dst  p\left(\hat{\rvx}_0 =\vx| {\hat {\rvx}_t = \vx_{a,t}}\right)$ to the true sample $\dst \vx_0$ with high probability.

% Then the resampled input $\hat{x_{0}}$ would be fed into classifier to get the predicted label. 


% \paragraph{Label majority voting numbers:}
% To perform our \name, label majority voting is important. Here we choose 40 as our majority voting numbers. In certification process, we need to implement such numbers of reverse process to each specific image after adding a Gaussian noise. Then we put these purified images through a classifier and choose the largest label cluster in the prediction label results as the final result of once certification sampling.


==> sections/method_bak2.tex <==
\section{\name }
Based on the theoretical analysis introduced before, it inspires us to propose the robust framework, \name. In this section, we will introduce \name and show how to calculate the  certified robustness via randomized smoothing algorithm. 
% Since it is hard to find the density region, here we empirically leverage the majority vote to estimate it.  
\paragraph{Framework. }
Our framework, \name,  consists of two components: (1)  an off-the-shelf diffusion model $f$ and (2) a classifier $h$ trained on the standard clean dataset (e.g. ImageNet).
Given an adversarial input, \name incorporates two steps for adversarial robustness. First, we feed the adversarial input into  the reverse process of the diffusion model to obtain a posterior data distribution conditioned on the input adversarial example. Second, we perform the reverse process multiple times to approximate the label with high density manifold via majority vote. 
% Given an adversarial input, \name incorporates two steps for adversarial robustness. First, we feed the adversarial input into  the reverse process of the diffusion model to obtain a posterior data distribution conditioned on the input adversarial example. Second, we take the point with the highest density in the obtained distribution as the purified sample. 
% Note that  as we have shown before, diffusion process itself is not necessary when leveraging diffusion models for adversarial purification. Instead, by sending the adversarial example directly through the reverse process of the diffusion model, we can obtain a better-recovered sample in terms of its distance to the corresponding clean sample. Thus, \name indeed removes the diffusion process of the diffusion model in our pipeline. 



% Note that here, we do remove the diffusion process of the diffusion model, instead,  by sending the adversarial example directly through the reverse process of the diffusion model. Our following theorem shows that we can obtain a better-recovered sample in terms of its distance to the corresponding clean sample
% \chaowei{Give a proof.}



When applying the above steps in practice, One challenge is that find the point with the highest density in the obtained distribution since it requires an enormous amount of samplings to confidently estimate the densities in the whole sample space.  For diffusion model, it is already quite expensive to even do sampling once. Thus, it is almost impossible to find such the point. 
% Because we need a huge amount of
% samplings to makes a confidential estimation of the densities for all points in the sample space. For
% diffusion model, it is quite expensive to even do sampling once.
To address it,  we approximate  the second step with \textit{majority vote} to reduce the heavy computation. Specifically,  if we only focus on classification, we first repeatedly send the scaled perturbed sample $\dst \vx_{a,t}$ through the reverse process of the diffusion to obtain multiple reversed samples and feed them into the classifier
to get the predictions. Then we use the majority vote on such predictions to provide the final label assigned to $\dst \vx_a$. 
% When most of the samples surround the true sample $\dst \vx_0$, we can say the label majority vote will give the label of the highest density point with high probability. \chaowei{@zhongzhu}

\paragraph{Certified Robustness with \name}
% First, similar to \citet{carlini2022certified}, our framework first map the randomized smoothing noise $\sigma$ to the noise used for the forward process of the diffusion model. Specifically, given a randomized smoothing parameter $\sigma$ and data input example $x$, randomized smoothing adds a Gaussian noise $\epsilon$, where $\epsilon \sim \mathcal{N}(0, \sigma^2 I)$ to $x$. We could directly map randomized example $x_{\text{rs}} = x+\epsilon$ with the forward processing of the diffusion model $x_\text{rs} = x_t \sim \mathcal{N}(\sqrt{\alpha_t} x_0, (1-\alpha_t) I) $  as :   
% \begin{equation*}
%     \sigma^2 = \frac{1-\alpha_t}{\alpha_t}
% \end{equation*}
% In this way, it equals to  calculate the corresponding timestep $t$ to satisfy the above equation. \chaowei{@jiongxiao, transfer it to SDE. }
Here, we show how to use Randomized Smoothing (RS)\citep{Cohen2019ICML} to calculate the certified robustness of \name. We follow the similar process of \citet{carlini2022certified}. Specifically, our framework first calculate the $t$, the step used for reverse process of diffusion model. To calculate it, given a  Gaussian noise $\epsilon \sim N(0, \sigma^2I)$,  randomized smoothing adds $\epsilon$ to data input $x$ to get the randomized data input $x_\text{rs} = x+\epsilon$. Thus, we map the randomized example $x_\text{rs}$ to data $x_t$ with $t$ step diffusion processing, where $x_t \sim \sqrt{\alpha_t}\mathcal{N}(x_0, \frac{1-\alpha_t}{\alpha_t} I)$ so that $\sigma^2 = \frac{1-\alpha_t}{\alpha_t}$.
In this way, we could directly compute $\alpha_t$ as:
    $\alpha_t = \frac{1}{1+\sigma^2}$
    

After that, we can get the corresponding $t$ of SDE by solving the following equation based on the selected schedule $\beta(t)$:
\begin{equation*}
    \alpha_t = e^{-\int_0^t\beta(s)ds}
\end{equation*}
Note that for discrete $\beta(t)$ schedule, we choose the timestep $t$ which makes the value of  $\frac{1}{1+\sigma^2}$ in the set $\left\{\sqrt{\alpha_s} | s=1...T \right\}$ nearest to $\sqrt{\alpha_t}$ .


Second, given the timestep $t$, we scale the  randomized smoothing sample $x_{rs}$ with  $\sqrt{\alpha_t}$ to get the scaled randomized smoothing sample $\sqrt{\alpha_t} x_{rs}$. We repeatedly feed the scaled randomized smoothing sample $\sqrt{\alpha_t} x_{rs}$  into the reverse processing of the diffusion $r$-times  to resample the reversed input $\{ \hat{x_{0}}^1 , \hat{x_{0}}^2, \cdots, \hat{x_{0}}^i,\cdots ,\hat{x_{0}}^r\}$, where $\hat{x_{0}}^i = \textbf{Reverse}( \sqrt{\alpha_t} x_{rs}, t)$. 
% As mentioned before, \name needs to locate the highest density point in the conditional distribution $\dst  p\left(\hat{\rvx}_0 =\vx| {\hat {\rvx}_t = \vx_{a,t}}\right)$ characterized by Theorem \ref{distribution:reverse}. 
% However, it is hard to do it in reality since we need a huge amount of samplings to makes a confidential estimation of the densities for all points in the sample space. It is extremely computational expensive in the high dimensional space. Thus, here we propose a simple but efficient strategy: \textit{majority voting}. 

Third, we feed the above reversed samples into a standard \emph{off-the-shelf} classifier to get the corresponding predicted labels $\{ h(\hat{x_{0}}^1), h(\hat{x_{0}}^2), h(\cdots, \hat{x_{0}}^i),\cdots ,h(\hat{x_{0}}^r\})$. We, then, apply \textit{majority vote}, denoted $\textbf{MV}({\cdots})$ on these predicted labels to get the final label for $x_{rs}$. 
% The algorithm also shows in Algo~\ref{}.

% \paragraph{Reduced  reverse sampling steps.}
For the reverse process of the diffusion model, it requires to repeatedly apply a ``single-step'' operation $t$ times to get the reversed sample  $x_{0}$ (i.e., $x_{0} = \underbrace{ \textbf{Reverse}( \cdots \textbf{Reverse}( \textbf{Reverse}(x_t; 1); 1); \cdots 1)}_{t \text{ steps}}$). Here $x_{t-1} = \textbf{Reverse}(x_t;1)$ means we  sample $x_{t-1} \sim \mathcal{N}(\widetilde{\mu}(x_t,x_0), \widetilde{\beta}_t I)$ with ``single-step'' operation, where
% \begin{equation*}
   $ \widetilde{\mu}(x_t,x_0) := \frac{\sqrt{\alpha_{t-1}}\beta_t}{1-\alpha_t}x_0 + \frac{\sqrt{\alpha_t}(1-\alpha_{t-1})}{1-\alpha_t}x_t$.
% \end{equation*}

However, using single step repeatedly to perform the whole $t$-step reverse process in the diffusion model is really time-consuming process. To reduce the time complexity, instead of using single step, here we reduce the repeatedly ``single-step'' reverse sampling processing with ``$b$-step ($b < t$)'' sparse sampling strategy by changing the reverse sampling schedule from $S^1 = \underbrace{ \{t, t-1, \cdots, 1\}}_{t}$ to $S^b = \underbrace{ \{t, t-\floor{\frac{t}{b}}, \cdots, 1 \}}_{b}$, where we fix the last step $t-b\floor{\frac{t}{st}}$ to 1, so that   $x_{0} = \underbrace{\textbf{Reverse}( \cdots \textbf{Reverse}( \textbf{Reverse}(x_t; \floor{t/b}]); \floor{t/b}]); \cdots ;\floor{t/b})}_{b \text{}}$. 
% \chaowei{The following needs to be changed! }


Within this context, for the new reverse sampling schedule $S^b = \{t, t-[\frac{t}{st}], \cdots, 1 \}$, we need to revise $\alpha_t$ to make it adapt to our reduced reverse sampling methods.Specifically,  we denote $S_i^b$ as the $i$-th element in $S^b$. We have the new noise schedule $\alpha_{S_i}$\chaowei{It is still unclear!}, which can be used to compute the following $\beta_{S_t}$ and $\widetilde{\beta}_{S_t}$:
\begin{equation*}
  \beta_{S_t} = 1 - \frac{\alpha_{S_t}}{\alpha_{S_{t-1}}},   \quad \widetilde{\beta}_{S_t} = \frac{1-\alpha_{S_{t-1}}}{1-\alpha_{S_t}}\beta_{S_t}
\end{equation*}
Then we can sample $x_{S^b_{i-1}} \sim \mathcal{N}(\widetilde{\mu}(x_{S^b_{i}},x_0), \widetilde{\beta}_{S^b_i} I)$ to speed up sampling with only $b$ steps.
% \begin{equation*}
%     \widetilde{\mu}(x_{S_{t}},x_0) := \frac{\sqrt{\alpha_{S_{t-1}}}\beta_{S_t}}{1-\alpha_{S_t}}x_0 + \frac{\sqrt{\alpha_{S_t}}(1-\alpha_{S_{t-1}})}{1-\alpha_{S_t}}x_{S_t}
% \end{equation*}




% If $st$ is too small,  $st$-step  sparse sampling strategy leads to a bad image quality after the reverse process. Thus, there exists a tradeoff to balance the quality and speed. 
% we finally use 10 steps during sampling. For fast sampling, we used Improving Sampling Speed method in \cite{}. 
% If the total number of sampling is $T$ steps, we can choose an arbitrary subsequence S of $1...T$ and do the reverse process just in t stpes, which is the length of subsequence S. For a give noise schedule $\overline{a}_t$, we can obtain the schedule $\overline{a}_{S_t}$, which is also a subset of $\overline{a}_t$. Then we will obtain sampling variances as
% \begin{equation*}
%   \beta_{S_t} = 1 - \frac{\overline{a}_{S_t}}{\overline{a}_{S_{t-1}}},   \quad \widetilde{\beta}_{S_t} = \frac{1-{S_{t-1}}}{1-{S_t}}\beta_{S_t}
% \end{equation*}
% Using such parameters, we can realize our reduced sampling steps. For the subsequence strategy, we simply do an equally partition to the total $T$ steps.


% We also find that larger sampling steps normally need more majority voting numbers to achieve their best results. This is because larger sampling steps will add more noise during reverse process. But the one step sampling method does not add any noise during reverse, so majority voting is not proper for one step method. 



% By using the majority vote strategy,when most of the samples surround the true sample $\dst \vx_0$, we can say the label majority vote will give the label of the highest density point with high probability. The following theorem is an adaptation of \cite[Theorem 3.2]{nie2022diffusion} bounding the distance of the samples in $\dst  p\left(\hat{\rvx}_0 =\vx| {\hat {\rvx}_t = \vx_{a,t}}\right)$ to the true sample $\dst \vx_0$ with high probability.

% Then the resampled input $\hat{x_{0}}$ would be fed into classifier to get the predicted label. 


% \paragraph{Label majority voting numbers:}
% To perform our \name, label majority voting is important. Here we choose 40 as our majority voting numbers. In certification process, we need to implement such numbers of reverse process to each specific image after adding a Gaussian noise. Then we put these purified images through a classifier and choose the largest label cluster in the prediction label results as the final result of once certification sampling.


==> sections/notations.tex <==
\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$  & A scalar (integer or real)\\
$\displaystyle \va$  & A vector\\
$\displaystyle \mA$  & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}


==> sections/tmp.tex <==

\subsection{Details about Fast Sampling}
\label{sec:fast}





% However, using single step requires running $n$ times reverse process in the diffusion model to get $\hat{\vx}_0$, which is a time-consuming process. 
Applying single-step operation $n$ times is a time-consuming process. In order
to reduce the time complexity, 
we follow the method used in ~\citep{nichol2021improved} and  sample a subsequence $S^b$ with $b$ values (i.e., $S^b= \underbrace{ \{n, \floor{n-\frac{n}{b}}, \cdots, 1 \}}_{b}$ 
% \kj{$\dst |S| = n, |S^b| = b$ if we need to save space later}
, where  $S_j^b$ is the $j$-th element in $S^b$ and $S_j^b=  \floor{n - \frac{jn}{b}}, \forall j < b \text{ and } S_b^b = 1$) from the original schedule $S$ (i.e., $S = \underbrace{ \{n, n-1, \cdots, 1\}}_{n}$, where $S_j= j $ is the $j$-th element in $S$).
% In this way, we reduce the sample schedule $s$  $n$  that the size of $S^b$ is $b$. 
% here we replace the $n$ times ``single-step'' reverse sampling process with %``$\floor{\frac{n}{b}}$-step ($b \ll n$)'' 
% $b$ times sparse reverse sampling strategy\citep{nichol2021improved} by changing the reverse sampling schedule from $S = \underbrace{ \{n, n-1, \cdots, 1\}}_{n}$
% ( where $S_j= j $ is the $j$-th element in $S$)  to 
% $S^b = \underbrace{ \{n, \floor{n-\frac{n}{b}}, \cdots, 1 \}}_{b}$ 
% % \kj{$\dst |S| = n, |S^b| = b$ if we need to save space later} 
% (where  $S_j^b$ is the $j$-th element in $S^b$ and $S_j^b=  \floor{n - \frac{jn}{b}}, \forall j < b \text{ and } S_b^b = 1$).


% $S_j^b = \floor{n - j\frac{n}{b}}$, is the $j$-th element in $S^b$  and the last step is fixed with 1). \kj{$S_j^b =  \floor{n - \frac{jn}{b}}, \forall j < b, S_b^b = 1$}
% (where  $S_j^b = \floor{n - j\frac{n}{b}}$, is the $j$-th element in $S^b$  and the last step is fixed with 1). \kj{$S_j^b =  \floor{n - \frac{jn}{b}}, \forall j < b, S_b^b = 1$}
% $t-b\floor{\frac{t}{b}}$ 
% , so that   $x_{0} = \underbrace{\textbf{Reverse}( \cdots \textbf{Reverse}( \textbf{Reverse}(x_t; \floor{\frac{t}{b}}]); \floor{\frac{t}{b}}]); \cdots ;\floor{\frac{t}{b}})}_{b}$ and $x_$
% \chaowei{The following needs to be changed! }


Within this context, 
% for the new reverse sampling schedule $S^b = \{t, t-[\frac{t}{st}], \cdots, 1 \}$, 
we adapt the original $\overline{\alpha}$ schedule $\overline{\alpha}^S$ = $\{\overline{\alpha}_1, \cdots, \overline{\alpha}_i, \cdots, \overline{\alpha}_n\}$ used for single-step to the new schedule $\overline{\alpha}^{S^b}$ = $\{\overline{\alpha}_{S_1^b}, \cdots, \overline{\alpha}_{S_j^b}, \cdots, \overline{\alpha}_{S_b^b}\}$ (i.e.,  $\overline{\alpha}^{S^{b}}_j = \overline{\alpha}_{S_j^b} = \overline{\alpha}_{S_{\floor{n - \frac{jn}{b}} }}$
is the $j$-th element in $\overline{\alpha}^{S^b}$).  
We calculate the corresponding $\beta^{S^b} = \{\beta^{S^b}_1, \beta^{S^b}_2, \cdots, \beta^{S^b}_j, \cdots,\beta^{S^b}_b  \}$ and $\widetilde{\beta}^{S^b} = \{ \widetilde{\beta}^{S^b}_1, \widetilde{\beta}^{S^b}_2, \cdots, \widetilde{\beta}^{S^b}_j, \cdots, \widetilde{\beta}^{S^b}_b \}$ schedules, where
% \begin{equation*}
 $ \beta_{S^b_j}=\beta^{S^b}_j = 1 - \frac{\overline{\alpha}^{S^{b}}_j }{\overline{\alpha}^{S^{b}}_{j-1}},   \quad \widetilde{\beta}_{S^b_j}=\widetilde{\beta}^{S^{b}}_j = \frac{1-\overline{\alpha}^{S^{b}}_{j-1}}{1-\overline{\alpha}^{S^b}_{j}}\beta_{S^b_j}$.
% \end{equation*}
With these new schedules,  we can use $b$ times reverse steps to  calculate   
$\hat{\vx}_{0} = \underbrace{\textbf{Reverse}( \cdots \textbf{Reverse}( \textbf{Reverse}(\vx_n; S^b_b); S^b_{b-1}); \cdots ; 1)}_{b}$.
% with only $b$ times.
Since $\boldsymbol{\Sigma}_{\boldsymbol{\theta}} (\vx_{S^b_{j}}, S^b_{j})$ is parameterized as a range between $\beta^{S^b}$ and $\widetilde{\beta}^{S^b}$, it will automatically be rescaled. Thus, $\hat{\vx}_{S^b_{j-1}} =  \textbf{Reverse}(\hat{\vx}_{S^b_j}; S^b_j) $  is  equivalent to sample
$\vx_{S^b_{j-1}}$ from $\mathcal{N}(\vx_{S^b_{j-1}}; \boldsymbol{\mu}_{\boldsymbol{\theta}} (\vx_{S^b_{j}}, S^b_{j}), \boldsymbol{\Sigma}_{\boldsymbol{\theta}} (\vx_{S^b_{j}}, S^b_{j}))$.
% \kj{The $\boldsymbol{\mu}_{\boldsymbol{\theta}}$ and $\boldsymbol{\Sigma}_{\boldsymbol{\theta}}$ were previously used for single time-step reverse, and they could also be used for a larger time step reverse? Or they should be a composition/recursion of themselves multiple times?}



